Learning Security Classifiers with Verified Global Robustness Properties

Many recent works have proposed methods to train classifiers with local robustness properties, which can provably eliminate classes of evasion attacks for most inputs, but not all inputs. Since data distribution shift is very common in security applications, e.g., often observed for malware detection, local robustness cannot guarantee that the property holds for unseen inputs at the time of deploying the classifier. Therefore, it is more desirable to enforce global robustness properties that hold for all inputs, which is strictly stronger than local robustness. In this paper, we present a framework and tools for training classifiers that satisfy global robustness properties. We define new notions of global robustness that are more suitable for security classifiers. We design a novel booster-fixer training framework to enforce global robustness properties. We structure our classifier as an ensemble of logic rules and design a new verifier to verify the properties. In our training algorithm, the booster increases the classifier's capacity, and the fixer enforces verified global robustness properties following counterexample guided inductive synthesis. We show that we can train classifiers to satisfy different global robustness properties for three security datasets, and even multiple properties at the same time, with modest impact on the classifier's performance. For example, we train a Twitter spam account classifier to satisfy five global robustness properties, with 5.4% decrease in true positive rate, and 0.1% increase in false positive rate, compared to a baseline XGBoost model that doesn't satisfy any property.

==> discussion.tex <==
\section{Discussion and Future Work}

\paragraph{More properties.}

\paragraph{Scale to larger datasets and models.}
Improve performance.


==> logicmodel.tex <==
\section{Logic Ensemble}

We propose a new type of classification model using ensemble of
logic rules, namely logic ensemble.
We design the model in a way such that it is
more expressive than the ensemble of trees, yet it preserves
explainability for an individual clause.
Therefore, the model has more capacity to learn the model-level properties.
Currently we focus on binary classification, but it can be extended to multi-class.

\subsection{Model Representation}

We propose the model $f(x)$ in the form of an ensemble of logical clauses,
where the input is a $d$-dimensional feature vector, $x = [x_1, x_2, ..., x_d]$.
A user can specify the number of clauses $N$, and the number of atoms in each clause $M$.
The output of the model is $f(x) = \sum_{k=1}^{N}{l_k}$, which sums up the activation value $l_k$
from all $N$ clauses. In particular, we use $C_k$ to represent the $k$-th clause, which is defined as the following.

$C_k \equiv ((\underset{i=1}{\overset{M}{\land}} t_i) \land l_k=a_k) \lor ((\lnot \underset{i=1}{\overset{M}{\land}} t_i) \land l_k=0)$, where \\
(1) $t_i \equiv \sum{w_j*x_j}$ compared to $\eta_i$, or \\
(2) $t_i \equiv $ logical formula of existing atoms and clauses.

The ensemble sums up the activation values from all clauses
to be the prediction score, i.e., $f(x) = \sum_{k=1}^{N}{l_k}$.
The activation value $l_k$ of each clause $C_k$
represents the vote from the clause. If the conjunction of atoms
over features evaluates to true (i.e., $\underset{i=1}{\overset{M}{\land}} t_i$ is true),
the activation value is either a positive or negative value representing
the vote towards malicious/benign class ($l_k=a_k$); otherwise the activation value
is zero ($l_k=0$). The model essentially aggregates the voting results from
individual clauses to make a final prediction.

Each atom in the clause can be sampled from some templates,
which specify domain knowledge in the structure of the atoms.
We only consider linear relationships among features in the atom, which has
the general form of $\sum{w_j*x_j}$ as the left-hand side term in comparison to a split threshold $\eta$.
If we use a naive template, we can include all the individual
features in the template separately, and let each atom randomly choose a feature and
the inequality ($<$ or $\geq$). This can generate atoms in the form $w*x_j < \eta$
or $w*x_j \geq \eta$, where $w$ and $\eta$ are learnable parameters.
We can also specify the inequality, the weight $w$, and/or the threshold $\eta$
if we have enough domain knowledge. For example, we can specify $x_1+x_2 < 10$ as
a template atom, if these two features are related and the sum smaller than 10 indicates
a prediction based on domain knowledge. In this case, the atom does not have learnable parameters.
To extend the types of atoms, an atom can be constructed using some existing clauses,
e.g., the negation of a clause.
Unless specified by the template, all the weights, thresholds, and clause activation values ($w, \eta, a$)
are learnable parameters.

\begin{comment}
\subsection{Robustness by Construction}

We want to give some guidance to the structure of the logic model
in order to learn robustness properties.

For filer type properties, Property 1 and 2, we adopt the same approach to encode the precondition
in the clauses of the logic model. Since $p \Rightarrow q$ is equivalent to $\lnot p \lor q$, we want to
encode the clauses into two cases, (1) $p \land q$,  and (2) $\lnot p$ with other atoms, where they both
satisfy the property. First, we assign a clause that
satisfies the precondition as $(p \land l_k=a_k) \lor ((\lnot p) \land l_k=0)$.
The activation value $l_k=a_k$ will be constrained by the meaning of $q$.
If the property says that the model should classify certain inputs as malicious,
we add the constraint that $a_k > 0$, which can be extended to an arbitrary range
of the activation value. For example, if the malicious filter set $M_0 = {1}$, we can specify $p$ as $x_0 \leq 1 \land x_0 \geq 1$, and constrain activation value $a_k > 0$.
For every other clause, we add $\lnot p$ as one of the atoms
in the definition of the logic model. By doing so, we want the model to learn the value of the vote
that strictly satisfy the precondition of the property, and we also want the model to learn
to classify data when the property precondition $p$ is false.

To extend the filter, when we don't know the exact set $M_j$, we can replace $p$ as $\tilde{p}$
in the clause construction to allow more learnable parameters.
For example, we can set the inequality of the atom structure
as $w_1x_1 > \eta_1$, when we know the inequality $>$ is preferred, but we don't specify the parameters $w_1$ and $\eta_1$.
The training process will learn these parameters as a way to learn the filtering set $M_j$.
The filter property and its variations are trivial to learn.

%We don't specify clause structure for Property 2a.

Property 3 is our first non-trivial property. We don't have a good idea how to construct the clauses yet.
Our intuition is that if there are more clauses using
as many features are possible, it is more likely to satisfy Property 3.
By luck, we have trained classifiers that satisfy property 3, through sampling
10 or 20 clauses with random feature and inequalities. This approach is ``guess-and-check''.
It explores too much of the model hypothesis space, so it is inefficient.

Haven't experimented with property 4 and 5 yet.


\subsection{Regular Training}

After we have the structure of the model through a combination of templates and sampling,
we use Continuous Logic Networks~\cite{ryan2019cln2inv} to smooth and train the model.
Following Ryan et al.~\cite{ryan2019cln2inv}, we use a shifted and scaled sigmoid function
to smooth the inequalities, product t-norm and product t-conorm to smooth conjunctions and disjunctions.
In the smoothed version, we use the additional constraints for weights and activation values related to
properties to guide the model learn these parameters if they are specified.
To train the smoothed model, we construct the loss as the binary cross-entropy loss for
classification, and minimize the loss using stochastic gradient descent.
After training, we discretize the model back to SMT formula for prediction, so we can certify the robustness properties.
In our experiments, the discrete version and the smoothed version of the model after training
have the same test accuracy.
\end{comment}

%What does domain knowledge stand for?
%\begin{itemize}
%	\item What represents maliciousness, e.g., monotonicity.
%	\item low-cost features, e.g., allowable perturbation range for different features.
%	\item basic units of attack operations
%\end{itemize}
%
%Some properties are unrelated to domain knowledge, but should
%make sense for robustness in general.



==> smtattack.tex <==
\section{Model Diagnosis}

Though decision trees are considered to be explainable,
in ensembles, the aggregation of rules have lost the explainability.
We provide a new method to diagnose tree ensemble models.

\subsection{Symbolic Property Attacks}

We would like to diagnose whether a trained tree ensemble classifier satisfies assumptions
made by security experts. These assumptions can be explicit or implicit, which are usually
the domain knowledge used in the feature engineering process. Ideally, the classifier should be consistent
with such domain knowledge. We propose a new SMT attack against trees to formally
check whether this is true. First, we encode tree models into a Satisfiability Modulo Theory (SMT) formula.
Then, we propose model properties by formally represent security domain knowledge using first order logic.
We translate the violations of properties into constraints, along with the constraints of the trees,
into a \emph{property violation formula}.
After that, we check the satisfiability of all the constraints for violating each property.
If the property violation formula is satisfiable (SAT), then we say the classifier $\mathcal{C}$
does not satisfy the property $\mathcal{P}$, i.e., $\mathcal{C} \not\models \mathcal{P}$.
On the contrary, if the property violation formula is unsatisfiable (UNSAT), then the classifier
satisfies the property, i.e., $\mathcal{C} \models \mathcal{P}$.
In our experiments, we use \texttt{Z3}~\cite{de2008z3} to solve the property violation formula.

\subsubsection{Boolean Encoding}





\subsubsection{Tree Ensemble Model Encoding}

%\begin{comment}
%\begin{figure}[t!]
%	\centering
%	\includegraphics[width=0.9\columnwidth]{figures/dnf.png}
%	\caption{An example for encoding tree ensembles into SMT formula. We represent each decision tree as a DNF. The tree ensemble
%	prediction is the sum of all leaf variables $l_i$.}
%	% the figure should be equality constraints, not assignment
%	\label{fig:dnf}
%\end{figure}
%\end{comment}

We encode each decision tree in the ensemble into a Disjunctive Normal Form.
The variables in the DNF formula are the input feature variables
and leaf variables. 
Specifically, we encode each path from the root
to a leaf in the decision tree as an AND clause. There are two types
of atoms in the clause: predicates and leaf nodes.
Every predicate in the path is an atom in the clause.
In addition, all leaf nodes have an atom in the clause, to indicate
that only one leaf variable can have a non-zero value at a time.
The leaf variable in the current path equals to the corresponding
leaf value in the decision tree, and all the other leaf variables
should equal to zero in the AND clause. After we have the AND clauses
for all the paths in a tree, we take the OR of them
as the DNF for the tree, since only one path can be taken during
prediction. The output of the tree ensemble is the sum
of all leaf variables from all the trees.

Figure~\ref{fig:dnf} shows an example of how to encode
the decision tree $f_1(x)$ into a DNF. There are two non-leaf
nodes, representing four predicate atoms: ``age $< 15$'', ``age $\geq 15$'',
``is male'', and ``is not male''. There are three paths in the tree,
and therefore we have three conjunctions in the OR clause.
Note that the leaf variable assignments within each conjunction
enforces the constraint that only one leaf variable can be activated
while the other leaf variables are zero in a given path.
We can encode $f_2(x)$ in the same way. The tree ensemble output is
$f(x) = l_1 + l_2 + l_3 + l_4 + l_5$. Given the DNF encoding, we
can conduct various attacks constrained by domain knowledge,
and to check whether a tree model satisfy some properties.

\begin{comment}

\red{The following properties are good to check. but not enough as goals to train.}

\textbf{Property 6 (single feature filter): } For a given feature j and its malicious
set $M_j$, $\forall x \in D_x, x_j \in M_j \Rightarrow f(x) \geq 0$

For any valid data input $x$, if a feature with strong domain knowledge $x_j$ is in
a restricted malicious value set $M_j(x)$, then the classifier
always outputs malicious prediction $f(x) \geq 0$.

\textbf{Property 7 (multi-feature filter):} For a set of features $J$
and their malicious set $M_{j} (j \in J)$, $\forall x \in D_x, \forall j \in J, x_{j} \in M_{j} \Rightarrow f(x) \geq 0$

This property extends Property 1 for multiple features.
Security experts usually have an idea about what is considered to be
the most malicious behavior if multiple features fall into some specific
value ranges.

\textbf{Property 7a (relaxed multi-feature filter):} For a set of features $J$
and their malicious set $M_{j} (j \in J)$, $\forall x \in D_x$, for all but one $M_j, x_j \in M_j(x) \Rightarrow f(x) > 0$.

This property relaxes the Property 7 by one feature dimension.

%\textbf{Property 4:} $\forall x \in D_x$, if we only know the value
%of $x_j \Rightarrow \max f(x) > 0$ and $\min f(x) < 0$.

\textbf{Property 8 (lack-of-evidence):} $\forall x \in D_x$, only knowing $x_j = a \Rightarrow \max f(x) \ge 0$ and $\min f(x) < 0$.

This property specifies that no single feature value can determine
whether something is benign or malicious, except in the cases
determined in Property 1. It is a common assumption
in related work that knowing one feature value is not enough to make
a distinction between malicious and benign behaviors, but knowing
the values of multiple features can. However, many trained models
do not satisfy this property. If no single feature value determines whether a data point is benign,
this is a global robustness property that ensures minimal adversarial evasion distance
$L_0 > 1$ given even unseen data points outside the training
and testing sets.

%\red{We can sort the predicates for $x_j$, then if one is true, all other atoms
%on the same side will be true, and those on the other side will be false.
%This doesn't need a solver, but enumerating all the atoms is still time consuming? Is it?
%Do it per feature? If one feature is good, then we are good?
%Do it per clause? If atoms in this clause is good, then we fix the clause?
%Only knowing $x_j = a$ is equivalent to only knowing the truth values of atoms
%involving one feature $x_j$.}

\end{comment}


\subsection{Attack Constraints}

%\yizheng{This can be used to check properties, and also to start from a concrete
%data point to evade the model in the traditional sense.}

\subsubsection{Property Violation Constraints}
We have written the model-level properties in the form of implication,
$\forall x, p \Rightarrow q$, which is equivalent to $\forall x, (\lnot p) \lor q$.
If the model does not satisfy the property, there exists a counterexample
that violates the property, i.e., $\exists x, p \land \lnot q$.
Hence, to check the satisfiability of a property for a classifier, we add constraints $p \land \lnot q$
to the SMT encoding of the classifier as the \emph{property violation constraints},
and use a solver to find a satisfiable assignment. If the solver returns UNSAT,
the classifier satisfies the property.

\textbf{Misclassification constraint:} In particular, if we want to check if
any property related to malicious behavior is misclassified
as benign, we add a constraint to the SMT formula such that
$l_1 + l_2 + l_3 + l_4 + l_5 < 0$.


\subsubsection{Attack Cost Constraints}

In addition to checking violation of model-level properties,
we can also use the proposed SMT attack to find specific evasion instances by perturbing a malicious data point.
Our SMT attack is expressive because we can encode constraints related to
semantics of the dataset, utility of the attack, low suspiciousness, and other types of attack costs.
Assuming that the attack modifies a malicious data point $x$ to evade the classifier,
we propose the following constraints for a realistic attack.

\textbf{Semantics of the feature:} We propose constraints related to the semantic of features,
and dependencies among features given a specific dataset.
For example, since many classifiers often use
statistics (mininum, average, maximum) of some measure as multiple features, we want
to keep the dependencies among these features for the attack. As another example,
to evade a PDF malware classifier, the attack need to specify data points that are functional PDFs.

% For example,
%whether a feature takes non-negative values, and whether one feature
%is always larger than some other feature values. 

\textbf{Utility of the attack:} We assume that the attacker wants to preserve
the intended goals even after trying to evade the classifier. In the case of cryptojacking,
the attacker wants to mine enough coins to ensure a reasonable economic return,
therefore, the attacker may not want to reduce the work load too much that no longer
makes the operation profitable, which can be expressed as the sum of load features
to be at least over some threshold.

\textbf{Low suspiciousness:} As proposed in previous works~\cite{pierazzi2020problemspace,chen2017practical},
a successful evasion attack should not make any metric too suspicious such that it is easy to detect
and filter out the attack. For example, injecting noisy content should in general preserve distribution of
features in evasive malware variants~\cite{pierazzi2020problemspace} and evasive bots~\cite{chen2017practical}.

\textbf{Small neighborhood constraint:} 
We can also add the $L_p$-norm bound constraint to the evasive instances, as borrowed
from the definition of adversarial images.


